A Co-Matching Model for Multi-choice Reading Comprehension

Multi-choice reading comprehension is a challenging task, which involves the matching between a passage and a question-answer pair. This paper proposes a new co-matching approach to this problem, which jointly models whether a passage can match both a question and a candidate answer. Experimental results on the RACE dataset demonstrate that our approach achieves state-of-the-art performance.

==> related.tex <==
\section{Related Work}
\label{sec:rel}

Sequence matching model between a pair of sequences has been widely explored on the tasks of text entailment~\cite{dagan2006pascal,snli:emnlp2015}, answer selection~\cite{voorhees1999trec}, etc.. For the multi-choice reading comprehension task, a model for matching a triplet of sequences is needed. The common strategy to solve this problem is to convert it into sequence pair matching problem. One way is to simply concatenate the candidate answer to the question, and then match the new sequence with the passage~\cite{richardson2013mctest,yin2016attention}. Another way is  first matching one pair of sequences the matching representation of which will be further used to match the left sequence~\cite{lai2017race,eliminet,xu2017towards,Haichao18:aaai}. In this paper, we propose a new way to co-match the passage with the question and answer for multi-choice reading comprehension.



